How Should Diffusion Language Models Edit Code?

Code editing requires a model to decide where to make changes, generate the new content, and preserve everything else. We study how masked diffusion language models divide these responsibilities across four editing interfaces: whole-file rewriting, search-and-replace, locate-then-infill, and token-level editing. Experiments on CanItEdit reveal a composition gap: diffusion models can generate coordinated changes when the correct edit locations are supplied, but much of this capability is lost when those locations must be predicted. Access to the intact original code helps the model fill multiple edit regions, yet does not resolve the difficulty of selecting those regions. By varying the editable regions while holding the generation model and decoding procedure fixed, we identify two distinct requirements for successful editing: covering every required change and placing precise boundaries around it. Missing a required region prevents the corresponding change, while widening regions to ensure coverage can sharply reduce success by requiring unchanged code to be regenerated. A sentence-level Wiki editing probe shows the same qualitative gap between supplied and predicted locations beyond code. These findings show why strong infilling capability alone does not ensure reliable editing: the interface must expose all required changes while limiting regeneration of unchanged code.

==> sections/7-negative.tex <==
% Supporting negative results were moved to Appendix~\ref{app:failed}.


==> sections/9-limitations.tex <==
% The limitations are now integrated into the Scope paragraph of Section 7
% (sections/8-discussion.tex). Keep the scientific qualifications there.
% ICLR 2027 Author Guidelines checked 2026-09-24: no separate limitations
% section is required. https://iclr.cc/Conferences/2027/AuthorGuidelines


==> sections/statements.tex <==
\newpage
\subsection*{AI use statement}
We used generative AI tools to draft and edit prose, create or edit software code, format references, and improve readability. We did not use them to generate synthetic datasets, develop theoretical models, formulate mathematical claims, write proofs, or interpret results without author verification. The authors reviewed all AI-assisted work and take responsibility for the final text, claims, and artifacts.

\subsection*{Ethics statement}
This work studies diffusion-language-model training on public code-editing datasets and benchmarks. It involves no human subjects or private user data. Code-generation systems could be used to modify software in unintended ways; we study them as research interfaces for instructional editing and adhere to the ICLR Code of Ethics.

\subsection*{Reproducibility statement}
The main text and appendix specify the edit interfaces, training recipes, decoding settings, checkpoint identities, CanItEdit protocol, HumanEval-Infilling placement probe, composition routing, scaffold corruptions, and construction controls. They distinguish autonomous results from gold-location and gold-length diagnostics and document recipe confounds and external capability references.

